Efficient Learning of Interpretable Classification Rules

Machine learning has become omnipresent with applications in various safety-critical domains such as medical, law, and transportation. In these domains, high-stake decisions provided by machine learning necessitate researchers to design interpretable models, where the prediction is understandable to a human. In interpretable machine learning, rule-based classifiers are particularly effective in representing the decision boundary through a set of rules comprising input features. The interpretability of rule-based classifiers is in general related to the size of the rules, where smaller rules are considered more interpretable. To learn such a classifier, the brute-force direct approach is to consider an optimization problem that tries to learn the smallest classification rule that has close to maximum accuracy. This optimization problem is computationally intractable due to its combinatorial nature and thus, the problem is not scalable in large datasets. To this end, in this paper we study the triangular relationship among the accuracy, interpretability, and scalability of learning rule-based classifiers. The contribution of this paper is an interpretable learning framework IMLI, that is based on maximum satisfiability (MaxSAT) for synthesizing classification rules expressible in proposition logic. Despite the progress of MaxSAT solving in the last decade, the straightforward MaxSAT-based solution cannot scale. Therefore, we incorporate an efficient incremental learning technique inside the MaxSAT formulation by integrating mini-batch learning and iterative rule-learning. In our experiments, IMLI achieves the best balance among prediction accuracy, interpretability, and scalability. As an application, we deploy IMLI in learning popular interpretable classifiers such as decision lists and decision sets.

==> chapters/additional/explanation.tex <==
\subsection{Illustration of Incremental Learning}
%Step by step rule formulation for an example
	\label{sec:example}
	We illustrate  an interpretable rule generated by $ \IMLI $ with step by step formulation over partitions on iris dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/iris}}. Iris dataset has four attributes: sepal length, sepal width, petal length, and petal width. All feature values are scaled in centimeter. Iris dataset has three classes: Iris Setosa, Iris Versicolour, and Iris Virginica. We consider the binary problem of classifying Iris Versicolour  from the other two species: Setosa and Verginica. Here we consider that $ \R $ is a single clause  DNF rule and learned over four partitions (e.g. $ \R_1, \dots, \R_4 $). The final rule $ \R $  is equivalent to $ \R_4 $. 
	
%	At first, we show $ \R_\MLIC $, the interpretable rule generated by $ \MLIC $ on the same parameter setting.
%	\begin{equation*}
%	\begin{split}
%	&\R_\MLIC:=\text{sepal width} \le 3.2 \,\wedge \, \text{petal length} \le 5.0 \,\wedge \, \\ 
%	& \qquad \qquad \quad\text{petal length} > 1.7\,\wedge \, \text{petal width} \le 1.5
%	\end{split}
%	\end{equation*}
	


\begin{equation*}
\begin{split}
&\R_1:=\text{petal length} \le 5.32 \,\wedge \, \text{petal length} > 1.7 \,\wedge \, \\
&\qquad\;\;\;\text{petal width} \le 1.8\\
&\R_2:=\text{sepal width} \le 3.1 \,\wedge \, \text{petal length} \le 5.32 \,\wedge \,\\ &\qquad\;\;\;\text{petal length} > 1.7 \,\wedge \, \text{petal width} \le 1.5\\
&\R_3:=\text{sepal width} \le 3.1 \,\wedge \, \text{petal length} \le 5.0 \,\wedge \,\\ &\qquad\;\;\;\text{petal length} > 1.7 \,\wedge \, \text{petal width} \le 1.5\\
& \R:=\text{sepal width} \le 3.1 \,\wedge \, \text{petal length} \le 5.0 \,\wedge \,\\ &\qquad\;\;\;\;\;\;\;\text{petal length} > 1.7 \,\wedge \, \text{petal width} \le 1.8
\end{split}
\end{equation*}
$ \R $ can be interpreted as: 
	a sample which satisfies all of the four constraints is predicted as Iris Versicolour. Here the  rule size $ | \R|=4 $. Specifically, $ \R_1 $ is learned on the first partition of training data. $ \R_2 $ learns two literals ($ 2^{nd} $ and $ 3^{rd} $) which also appear in $ \R_1 $, introduces two new literals ($ 1^{st} $ and $ 4^{th} $) while learning on the second training partition, and falsifies a previously learned literal  from $ \R_1 $ (i.e., $ (\text{petal width} \le 1.8 $). 
	
	Since the dataset contains continuous valued features, $ \IMLI $ removes redundant literals at each step of learning by applying  Algorithm \ref{alg:imli-RRL}. For example, we show the  generated rule $ \R_3' $  for the $ 3^{rd} $ partition if we do not apply Algorithm \ref{alg:imli-RRL}. 
	
	
%	 ($ 1^{st} $, and $ 2^{nd} $ literal). $ \R_2 $ does not contain the $ 3^{rd} $ literal of $ \R_1 $ because $ \IMLI $ learns $ \sigma_2(\text{petal width} \le 1.8)=0 $. Note that the $ 1^{st} $ literal of $ \R_2 $ is not in $ \R_1 $ but appears in $ \R_2 $.  We notice that initial learned rule is shorter in length (e.g., $ |\R_1|=3 $), however, as we learn rule for more training batches, rule size increases (e.g., $ |\R_2|=|\R_3|=|\R_4|=4 $). 
%
%\begin{equation*}
%	\begin{split}
%	&\R_1':=\text{petal length} \le 5.32 \,\wedge\, \text{petal length} > 1.7 \,\wedge\,\\
%	 &\qquad\;\;\;\text{petal width} \le 1.8\\
%	&\R_2':=\text{sepal width} \le 3.1 \,\wedge\, \text{petal length} \le 5.32 \,\wedge\,\\
%	 &\qquad\;\;\;\text{petal length} > 1.7 \,\wedge\, \text{petal width} \le 1.5 \,\wedge\,\\
%	  &\qquad\;\;\;\underline{\text{petal width} \le 1.8}\\
%	&\R_3':=\text{sepal width} \le 3.1 \,\wedge\, \text{petal length} \le 5.0 \,\wedge\, \\
%	&\qquad\;\;\;\underline{\text{petal length} \le 5.32} \,\wedge\, \text{petal length} > 1.7 \,\wedge\, \\
%	&\qquad\;\;\;\text{petal width} \le 1.5 \,\wedge\, \underline{\text{petal width} \le 1.8}\\
%	&\R_4':=\text{sepal width} \le 3.1 \,\wedge\, \text{petal length} \le 5.0 \,\wedge\, \\
%	&\qquad\;\;\;\underline{\text{petal length} \le 5.32} \,\wedge\, \text{petal length} > 1.7 \,\wedge\, \\
%	&\qquad\;\;\;\text{petal width} \le 1.8
%	\end{split}
%\end{equation*}
%	

\begin{equation*}
\begin{split}
&\R_3':=\text{sepal width} \le 3.1 \,\wedge\, \text{petal length} \le 5.0 \,\wedge\, \\
&\qquad\;\;\;\underline{\text{petal length} \le 5.32} \,\wedge\, \text{petal length} > 1.7 \,\wedge\, \\
&\qquad\;\;\;\text{petal width} \le 1.5 \,\wedge\, \underline{\text{petal width} \le 1.8}\\
\end{split}
\end{equation*}

	The underline marked literals are redundant, hence removed in $\R_3 $.






==> chapters/additional/improvement.tex <==
\section{Extra... previous}
\section{Improving the baseline}

\begin{comment}
		\begin{itemize}
		\item The number of clauses in the MaxSAT query is $ \mathcal{O}(k \cdot m \cdot n) $. We want to reduce the query size by addressing all the dependent parameters. 
		\item Learning single clause rule is easier than learning a multi-clause rule. 
		\item 
		\item We adopt mini-batch learning where we consider a reduced number of samples generated i.i.d. from the original training data. Since want to learn the value of discrete decision variables and the cost function is non-differentiable, it is tricky (may be impossible) to learn the optimum value because no convergence guarantee is available for discrete problem.  We propose a solving technique where we modify the value of a decision variable only if it tries to  optimize the cost function.
		
		\end{itemize}
		\begin{theorem}
		If a  training  sample   is predicted false by clause $ C_l $ in the $ l $-th iteration, the sample is also be predicted false by a CNF formula including clause $ C $. 
		Therefore,  the sample  can be removed from the training set while learning $ C_{l+1} $.
		\end{theorem}
		
\end{comment}

In this section, we discuss how to improve the  proposed MaxSAT formulation in Section~\ref{sec:encoding}. In particular, we discuss how to reduce both the  number of variables and the number of clauses in the formulation. The complexity of the MaxSAT query depends on three factors: the number of binary features $ m $,  the number of clauses  $ k $ in the desired rule, and the size of the  training set $ n $.    Therefore, we propose to (i)  rank features based on their contribution to the correctness in prediction and consider only more important features in Section~\ref{sec:feature_elimination}, (ii)  learn a single clause rule iteratively on a reduced training set in Section~\ref{sec:iterative_learning}, and (iii) learn rules in  a novel incremental  mini-batch approach tailored for  the discrete optimization problem in Section~\ref{sec:incremental_learning}.  Finally  in Section~\ref{sec:all_hypotheses}, we  discuss an improved formulation that takes benefit of all three proposed hypotheses. 


\subsection{Feature Ranking}
\label{sec:feature_elimination}

	All features in the training dataset do not contribute similarly in the prediction and thus do not appear in rule $ \Rule $. In the following, we  rank features based on their individual contribution to the accuracy of $ \Rule $ and propose to  formulate the MaxSAT query with higher ranked features. \red{cite dmitry and show difference}
	
%	We rank features with the assumption that $ \Rule $ is a single clause rule and empirically show that this assumption does not affect the prediction accuracy of multi-clause rules.
	We rank features considering both feature-value and  class label of samples in the training set. For the $ j $-th feature, we measure the number of  positive labeled samples having feature-value $ 1 $ (denoted as $ \mathsf{TP}_j $) and the number of  negative labeled samples having feature-value $ 1 $ (denoted as $ \mathsf{FP}_j $) in the training set $ (\mathbf{X}, \mathbf{y}) $.
	\[
	\begin{split}
		 &\mathsf{TP}_j= \sum_{i=1}^{|\mathbf{X}|} \mathds{1}_{y_i=1 \;\wedge\; \mathbf{X}_{i,j}=1}\\
		 &\mathsf{FP}_j= \sum_{i=1}^{|\mathbf{X}|} \mathds{1}_{y_i=0 \;\wedge\; \mathbf{X}_{i,j}=1}
	\end{split}
	\]
	
	
	 In order to rank  features based on their individual contribution  to the prediction accuracy, we use $ \mathsf{TP}_j -\mathsf{FP}_j $ as the ranking metric such that features with higher value of $ \mathsf{TP}_j -\mathsf{FP}_j $ have higher rank.  Avoiding notational clutter, we overload $ \mathsf{TP}_C $ and $ \mathsf{FP}_C $  on a  disjunction of features in the  clause $ C $ as follows.
	
	
	\[
	\begin{split}
	&\mathsf{TP}_C= \sum_{i=1}^{|\mathbf{X}|} \mathds{1}_{y_i=1 \;\wedge\; (\bigvee_{j|b_j \in C}\mathbf{X}_{i,j}=1)}\\
	&\mathsf{FP}_C= \sum_{i=1}^{|\mathbf{X}|} \mathds{1}_{y_i=0 \;\wedge\; (\bigvee_{j|b_j \in C}\mathbf{X}_{i,j}=1)}
	\end{split}
	\]
	
	Exact computation of $ \mathsf{TP}_C $ and $ \mathsf{FP}_C $ is computationally expensive because one would require to find the disjunction of features in $ C $ for all samples. However, it is easier to find their upper bound $ \mathsf{UB}(\cdot) $ and  lower bound $ \mathsf{LB}(\cdot) $. In particular,  $ \mathsf{UB}(\mathsf{TP}_C) = \sum_{j|b_j \in C} \mathsf{TP}_j $, $ \mathsf{LB}(\mathsf{TP}_C) = \max_{j|b_j \in C} \mathsf{TP}_j $,  $ \mathsf{UB}(\mathsf{FP}_C) = \sum_{j|b_j \in C} \mathsf{FP}_j $, and $ \mathsf{LB}(\mathsf{FP}_C) = \max_{j|b_j \in C} \mathsf{FP}_j $.
	
	
	In the following, we show the justification of using $ \mathsf{TP}_j -\mathsf{FP}_j $ as the ranking metric.
	

	\begin{theorem}
		\label{theorem:ub_of_acc}
		Let $ C $ and $ C' $ be two clauses  differing in  one  feature, namely feature $ j $ and feature $ j' $ respectively, and $ \mathsf{TP}_j - \mathsf{FP}_j > \mathsf{TP}_{j'} - \mathsf{FP}_{j'} $. Then 
		$ \mathsf{UB}(\mathsf{TP}_{C}-\mathsf{FP}_{C}) > \mathsf{UB}(\mathsf{TP}_{C'}-\mathsf{FP}_{C'})  $.
	\end{theorem}
	

%	\end{theorem}
	
	\begin{proof}
		\red{need to rewrite}
		\label{proof:ub_of_acc}
		\[
		\begin{split}
		& \sum_{b_i \in C} \mathsf{TP}_i \ge \mathsf{TP}_C \ge \max_{i:b_i \in C}  \mathsf{TP}_i\\
		& \sum_{b_i \in C} \mathsf{FP}_i \ge \mathsf{FP}_C \ge \max_{i:b_i \in C}  \mathsf{FP}_i\\
		\end{split}
		\]
		Therefore, 
		\[
			\mathsf{TP}_C-  \mathsf{FP}_C \le 	\sum_{b_i \in C} \mathsf{TP}_i - \max_{i:b_i \in C}  \mathsf{FP}_i
		\]


		Now
		\[
		\mathsf{TP}_{C_{(j)}} -  \mathsf{FP}_{C_{(j)}} \le 	\sum_{b_i \in C} \mathsf{TP}_i - \max_{i:b_i \in C}  \mathsf{FP}_i \le \sum_{b_i \in C \wedge i\ne j} \mathsf{TP}_i + \mathsf{TP}_j- \mathsf{FP}_j 
		\]
		Similarly,
		\[
		\mathsf{TP}_{C_{(j')}} -  \mathsf{FP}_{C_{(j')}} \le \sum_{b_i \in C \wedge i\ne j'} \mathsf{TP}_i + \mathsf{TP}_{j'}- \mathsf{FP}_{j'} 
		\]
		Since $ \mathsf{TP}_j - \mathsf{FP}_j > \mathsf{TP}_{j'} - \mathsf{FP}_{j'} $, we  deduce following conclusion regarding the upper bound.
		\[
		\mathsf{UB}(\mathsf{TP}_{C_{(j)}}-\mathsf{FP}_{C_{(j)}}) > \mathsf{UB}(\mathsf{TP}_{C_{(j')}}-\mathsf{FP}_{C_{(j')}})
		\]
			\end{proof}
	
	\subsection{Feature Elimination}
	
	We refer to the  accuracy of a clause in $ \Rule $ as proportional to the difference between true positive and false positive samples covered by the clause. While constructing the MaxSAT query, we can eliminate a feature that cannot increase the accuracy of the clause in which it may be included. The following theorem states when to eliminate feature $ j $ depending on the value of $ \mathsf{TP}_j - \mathsf{FP}_j $ in the training set.
	
	
	
	\begin{theorem}
		Consider two clauses $ C $ and $ C_{(\setminus j)} $ such that $ C_{(\setminus j)} $ has all features of $ C $ except feature $ j $. If  $ \mathsf{TP}_j - \mathsf{FP}_j < 0 $, then  $ \mathsf{UB}(\mathsf{TP}_{C}-\mathsf{FP}_{C}) < \mathsf{UB}(\mathsf{TP}_{C_{(\setminus j)}}-\mathsf{FP}_{C_{(\setminus j)}}) $, and feature $ j $ can be eliminated.
	\end{theorem}


%	\begin{theorem}
%		Let $ C_{(j)} $ and $ C_{(\setminus j)} $ 
%		If   $ \mathsf{TP}_j - \mathsf{FP}_j < 0 $ for the $ j $-th feature, removing this feature will increase the upper bound on accuracy of a clause in a CNF rule.
%	\end{theorem}

	\begin{proof}
		From Proof~\ref{proof:ub_of_acc}
		\[
		\begin{split}
				&\mathsf{TP}_C -  \mathsf{FP}_C \le \sum_{b_i \in C \wedge i\ne j} \mathsf{TP}_i + \mathsf{TP}_{j}- \mathsf{FP}_{j} \\
		&\mathsf{TP}_{C_{(\setminus j)} } -  \mathsf{FP}_{C_{(\setminus j)} } \le \sum_{b_i \in C_{(\setminus j)}} \mathsf{TP}_i 
		\end{split}
		\]
		 Since $  \sum_{b_i \in C \wedge i\ne j} \mathsf{TP}_i  =  \sum_{b_i \in C_{(\setminus j)}} \mathsf{TP}_i $ and $ \mathsf{TP}_j - \mathsf{FP}_j < 0 $, then 
		\[
		\mathsf{UB}(\mathsf{TP}_{C}-\mathsf{FP}_{C}) < \mathsf{UB}(\mathsf{TP}_{C_{(\setminus j)}}-\mathsf{FP}_{C_{(\setminus j)}})
		\]
	\end{proof}

	\begin{remark}
		In the MaxSAT Query, feature $ j $ can be eliminated in two ways: (i) removing the column associated with feature $ j $ from the  training set and (ii)  adding a hard clause $ S_j^i:= \neg b_j^i , \forall i$ with weight $ \mathsf{wt}(S_j^i)=\infty $. 
	\end{remark}
	
	
\section{Iterative Clause Learning}
\label{sec:iterative_learning}
	
	We design an iterative clause learning technique motivated by the set covering algorithm, also known as  the separate-and-conquer algorithm in symbolic rule learning~\cite{furnkranz1999separate}.
	A separate-and-conquer algorithm searches for a clause that explains/covers a part of the training set, separates samples covered by the clause, and recursively conquers the samples by learning more clauses until no samples remain. A family of rule learning approaches share the same top-level outer loop of the separate-and-conquer algorithm.
	The major difference among all approaches  is how they learn individual clauses, and in this paper we learn individual clauses using the MaxSAT-based formulation. We organize this section as follows. We first discuss which samples to  eliminate in Section~\ref{sec:sample_elimination}, formulate the objective function for the iterative approach in Section~\ref{sec:obj_iterative}, discuss the MaxSAT encoding in Section~\ref{sec:encoding_iterative} and  the early terminating condition of the iterative approach in Section~\ref{sec:termination_iterative}. 
	
	\subsection{Sample Elimination}
	\label{sec:sample_elimination}
	In the MaxSAT formulation in Section~\ref{sec:encoding}, the number of clauses in the query is linear with the number of clauses $ k $ in the desired rule $ \Rule $. We can improve this formulation by learning one clause at a time for at most $ k $ times and then merge all clauses using Boolean conjunction. Since the learned rule is in conjunction with each other, at each iteration we remove samples that are predicted false by the learned clause. In the following, we show that the removed samples are also predicted false by $ \Rule $. 
	
	
	
	

	
	
		

	
	\begin{theorem}
		\label{theorem:sample_remove}
		In the iterative clause learning approach, let $ \Rule $ be the learned rule and  $ \clause(\Rule,t) $ be the learned clause at the $ t $-th iteration. Let $ \mathbf{x}  $ be the vector of  Boolean features of a sample and  $ \mathbf{x} $ is predicted false by $ \clause(\Rule,t) $, i.e., $ \bigvee_{j:b_j^t \in \clause(\Rule,t)} x_j=0 $.
		Then the prediction of $ \mathbf{x} $ by the rule  $ \R $ is false, i.e, $ \Rule(\mathbf{x}) = 0 $. 
	\end{theorem}
	\begin{proof}
		\red{rewrite}
		According to the the construction of a $ k $-clause CNF rule $ \Rule $, 
		
		\[
			\Rule(\mathbf{x})=\bigwedge_{i=1}^k \bigvee_{j:b_j^i \in \clause(\Rule,i)} x_j 
		\]
		\[
		\hat{y}(\mathbf{x})= \bigwedge_{i=1}^k \bigvee_{j=1}^m x_jw_{i,j}
		\]  
		
		Since $ (\bigvee_{j:b_j^t \in \clause(\Rule,t)} x_j)=0 $, we reach the following conclusion. 
		\[
		\begin{split}
		\Rule(\mathbf{x})&= \bigwedge_{i=1}^k \bigvee_{j:b_j^i \in \clause(\Rule,i)} x_j \\
		&=\bigvee_{j:b_j^t \in \clause(\Rule,t)} x_j \wedge  \bigwedge_{i=1, i \ne t }^k \bigvee_{j:b_j^i \in \clause(\Rule,i)} x_j \\
		&= 0 \wedge \bigwedge_{i=1, i \ne t }^k \bigvee_{j:b_j^i \in \clause(\Rule,i)} x_j\\
		&=0
		\end{split}
		\] 
		%			\[
%			\hat{y}(\mathbf{x})= \bigwedge_{i=1}^k \bigvee_{j=1}^m x_jw_{i,j}=(\bigvee_{j=1}^m x_jw_{r,j}) \wedge  \bigwedge_{i=1, i \ne r }^k \bigvee_{j=1}^m x_jw_{i,j}= 0 \wedge \bigwedge_{i=1, i \ne r }^k \bigvee_{j=1}^m x_jw_{i,j}=0
%			\] 
			\end{proof}
		
		
	
	\subsection{Objective Function}
	\label{sec:obj_iterative}
	 We now  define the objective function in the iterative approach. The major difference  in the objective function with Eq.~\ref{eq:obj} is that  the number of samples differs  in each iteration as we eliminate  a subset of samples that are predicted false by the learned clause. Let $ k $ be the number of clauses in the desired rule and clause $ \clause(\Rule,t) $ be learned  at the $ t $-th iteration.	Given a training set $ (\mathbf{X}, \mathbf{y})$ of size $ n $ with each sample having $ m $ binary features, let $ n_t $ be the size of the training set  at the $ t $-th iteration, where $ t=1, \dots, k $ and $ n_1=n $. Let $\mathcal{E}_{\clause(\Rule,t)} $ be the set of samples that are  predicted incorrectly by $ \clause(\Rule,t) $, i.e., $ \mathcal{E}_{\clause(\Rule,t)} = \{(\mathbf{X}_i,y_i) | y_i \oplus \bigvee_{j:b_j^t \in \clause(\Rule,t)} \mathbf{X}_{i,j}= 1 \} $.	Given the data-fidelity parameter $ \lambda $,  we optimize the following function at the $ t $-th iteration. 
	
	\begin{equation}
	\label{eq:obj_iterative}
	\min_{{\clause(\Rule,t)}} \quad \frac{\lambda}{n} \sum_{i=1}^{n_t}|\mathcal{E}_{\clause(\Rule,t)}| + \frac{(1-\frac{n_t}{n}\lambda)}{mk}|{\clause(\Rule,t)}|
	\end{equation}
 		
	
	The objective function in Eq.~\ref{eq:obj_iterative} ensures that the penalty on prediction error of a sample is  same in all iterations, which is $ \frac{\lambda}{n} $.  Since we emphasis the objective-value  to be $ 1 $ in the worst case as in Eq.~\ref{eq:obj},  the penalty on selecting a feature in the $ t $-th clause is set to $ \frac{(1-\frac{n_t}{n}\lambda)}{mk} $. As a  subset of training set is removed at each iteration ($ n_t \ge n_{t+1} $), the penalty on rule-sparsity monotonically increases as the iteration advances. As a result, the objective function prefers smaller clauses as we progress in the iterative approach. 
	
	\subsection{MaxSAT Encoding}
	\label{sec:encoding_iterative} 
	To learn clauses in the iterative approach, the MaxSAT query presented in Section~\ref{sec:encoding} has to be modified. The soft clauses $ E_q $ and $ S_j^i $ are kept same as in Eq.~\ref{soft_clause_error} and~\ref{soft_clause_feature} respectively while their weights are modified based on the co-efficients of prediction error and rule-sparsity in the objective function in Eq.~\ref{eq:obj_iterative}.  In particular, we set $ \mathsf{wt}(E_q)=\frac{\lambda}{n} $ and $ \mathsf{wt}(S^i_j)=\frac{(1-\frac{n_t}{n}\lambda)}{mk} $. Finally, we construct the hard clause $ H_q $ by setting $ k=1 $ in Eq.~\ref{hard_clause_rule_consistency} as we  learn one clause at each iteration. 
	
	\subsection{Terminating Condition:}
	\label{sec:termination_iterative}
	As our goal is to learn a $ k $-clause rule $ \Rule $, the presented iterative approach is repeated for at most $ k $ iterations. However, it is possible to terminate early if  $ \clause(\Rule, t) $ can not cover any new sample in the training set at the $ t $-th iteration. In that case, $ \clause(\Rule, t) $ is not included in $ \Rule $ and the iterative process terminates. We summarize our discussion in the following theorem. 
	
	
	\begin{theorem}
		\label{thm:iterative_termination}
		Let $ (\mathbf{X}, \mathbf{y}) $ be the training set and $ \clause(\Rule,t) $ be the learned clause at the $ t $-th iteration. If  all samples in $ (\mathbf{X}, \mathbf{y}) $ are predicted true (i.e, 1)  by $ \clause(\Rule,t) $, that is, $ \bigvee_{j:b_j^t \in \clause(\Rule,t)} \mathbf{X}_{i,j} =1, \forall i$, then $ \clause(\Rule,t) $ is not included in $ \Rule $ and the iterative approach terminates after iteration $ t $. 
	\end{theorem}
			
%	\begin{theorem}
%		Suppose clause $ \mathbf{w}_r $ is learned at the $ r $-th iteration. If $ \sum_{i=1}^{n_r} \mathds{1}_{\bigvee_{j=1}^mx_{i,j}w_{r,j}=0}=0 $, then $  \mathsf{w}_r $ is not included in classifier $ \hat{y} $ and the iterative process terminates.  
%	\end{theorem}
	
	\begin{proof}
		\red{rewrite}
		 According to Theorem~\ref{theorem:sample_remove}, $ (\mathbf{X}, \mathbf{y}) $ consists of samples that are predicted true by $ \clause(\Rule,t-1) $  learned at iteration $ t-1 $.  Since $ \forall i,  (\bigvee_{j:b_j^t \in \clause(\Rule,t)} \mathbf{X}_{i,j}) =1 $, $ \clause(\Rule,t) $ only covers ( i.e., predicts true) a sample that is also covered by $ \clause(\Rule,t-1) $. Therefore, $ \clause(\Rule, t) $ is redundant  and hence not included in $ \Rule $.
		 
		 
%		 Since $ \sum_{i=1}^{n_r} \mathds{1}_{\bigvee_{j=1}^mx_{i,j}w_{r,j}=0}=0 $,  all training samples are  predicted \emph{true} by $ \mathbf{w}_r $ and no sample is predicted \emph{false}. Therefore, all samples at iteration $ r $ is covered by $ \mathbf{w}_{r-1} $, hence $ \mathbf{w}_r $ is not included in the classifier rule.   
		
		Since $ \clause(\Rule, t) $ predicts all samples as true, $ (\mathbf{X}, \mathbf{y}) $ will also be the training set at iteration $ t+1 $ because no sample is removed (Theorem~\ref{theorem:sample_remove}). Therefore, the iterative approach will learn the same clause again, hence the approach can be terminated

\end{proof}		

	
	
%	\newcommand{\maxsatquery}{\ensuremath{\mathsf{ConstructQuery}}}
%	\newcommand{\createclause}{\ensuremath{\mathsf{ConstructClause}}}
%	\newcommand{\iterativeClauseLearning}{\ensuremath{\mathsf{IterativeClauseLearning}}}
%	\let\oldReturn\Return
%	\renewcommand{\Return}{\State\oldReturn}

	\begin{algorithm}
		\caption{Iterative  clause learning}
		\begin{algorithmic}[1]
			\Function{\iterativeClauseLearning}{$ \mathbf{X},\mathbf{y}  ,k,\lambda $}
			\State $ \Rule=\{\} $
			\For{$ t=1, \dots, k $} \label{alg:itr_for_start}
			\State $ Q,W\leftarrow \maxsatquery(\mathbf{X},\mathbf{y},\lambda) $ \label{alg:itr_constructQuery}
			\State $ \sigma^* \leftarrow \MaxSAT(Q,W) $  \label{alg:itr_MaxSATSolving}
			\State $ C \leftarrow \createclause(\sigma^*) $
			\label{alg:itr_createClause}
			\If{$ \bigvee_{j:b_j^t \in C} \mathbf{X}_{i,j} =1, \forall i$} \label{alg:itr_termination_check}
			\State break \label{alg:itr_terminate}
			\EndIf
			\State $\clause(\Rule, t)\leftarrow C $ \label{alg:itr_clauseAdd}
			\State $ (\mathbf{X},\mathbf{y}) =\{(\mathbf{x},y) \in (\mathbf{X},\mathbf{y})| \bigvee_{j:b_j^t \in \clause(\Rule,t)} \mathbf{x}_{j} = 1 \}  $ \label{alg:itr_removeSamples}
			\EndFor 
			\Return $ \Rule $ \label{alg:itr_for_end}
			\EndFunction
		\end{algorithmic}
	\label{alg:iterative}
	\end{algorithm} 

\subsection{Description of Algorithm}
We show the algorithm for iterative clause learning in Algorithm~\ref{alg:iterative}. The algorithm takes  in inputs as  the training dataset $ (\mathbf{X}, \mathbf{y}) $, the data-fidelity parameter $ \lambda $, and the number of clauses $ k $ in the desired rule   and outputs the learned rule  $ \Rule $. Initially $ \Rule $ is an empty rule. The main loop in the algorithm repeats for at most $ k $ times while learning one clause in each iteration (Line~\ref{alg:itr_for_start}--\ref{alg:itr_for_end}). Inside the loop, the function {\maxsatquery}  in Line~\ref{alg:itr_constructQuery}  constructs the MaxSAT query $ Q $ and the weight $ W $ of clauses in $ Q $ for the dataset $ (\mathbf{X}, \mathbf{y}) $ as described in Section~\ref{sec:encoding_iterative}. A MaxSAT solver takes in $ Q $ and $ W $ as inputs, solves the query and returns the optimal assignment $ \sigma^* $ (Line~\ref{alg:itr_MaxSATSolving}). Based on the assignment, function {\createclause} in Line~\ref{alg:itr_createClause} constructs a clause $ C $ as described in Construction~\ref{construction:rule}. Then the algorithm checks if the learned clause $ C $ can cover any new sample in the training set in Line~\ref{alg:itr_termination_check}. If  $ C $ does not cover any new sample, $ C $ is not added in Rule $ \Rule $ and the learning process terminates according to Theorem~\ref{thm:iterative_termination} (Line~\ref{alg:itr_terminate}), otherwise $ C $ is added in $ \Rule $ (Line~\ref{alg:itr_clauseAdd}). Finally, a subset of samples that are predicted false are removed from the training dataset (Line~\ref{alg:itr_removeSamples}) and then process repeats.
	
		
		
	
%	Let consider a simplified objective function in iterative learning. If we learn $ t $ clauses in $ t $ iteration, we find a classifier as follows. 
%	
%	\begin{equation}
%	\label{eq:obj_it}
%	\min_{w_{r,j}} \quad \lambda_1 \sum_{i=1}^{n}\frac{\eta_i}{n} +\lambda_2 \sum_{r=1}^t\sum_{j=1}^{m} \frac{w_{r,j}}{m \cdot t} 
%	\end{equation}
%	
	
%	\subsection{Terminating Condition}
%	Now we will discuss about the terminating condition of iterative learning. 
%	
%	As we have discussed earlier, a set of samples are removed at each iteration that are predicted \emph{false} by the new learned clause. At iteration $ t $, the removed set consists of both false negative ($ \mathsf{FN}_t $) and true  negative ($ \mathsf{TN}_t $) samples.  Therefore, in the remaining dataset, all negative examples are false positive ($ \mathsf{FP}_t $) and all positive examples are true positive ($ \mathsf{TP}_t $). Therefore, the objective value at iteration $ t $ can be computed as follows. 
%	
%	\[
%	z_t = \min_{w_{r,j}} \lambda_1 \frac{\mathsf{FP}_t+\sum_{i=1}^t\mathsf{FN}_i}{n} +\lambda_2 \sum_{r=1}^t\sum_{j=1}^{m} \frac{w_{r,j}}{m \cdot t} 
%	\]
%	
%	
%
%	
%%	In the above inequality,  we compare the minimum value of LHS ($ \mathsf{LHS}_{\min} $) and the maximum value of RHS  ($ \mathsf{RHS}_{\max} $) and if $ \mathsf{LHS}_{\min} < \mathsf{RHS}_{\max} $, we terminate. 
%%	To  get $ \mathsf{LHS}_{\min} $, we  set $ \sum_{j=1}^{m}w_{t+1,j} =m $. 
%%	Since  $   \mathsf{FP}_{t+1}+ \mathsf{FN}_{t+1} \le \mathsf{N}_{t+1}+ \mathsf{P}_{t+1} $, which is, the total number of false negative and false positive is at most the total number of positive and negative samples, $ \mathsf{RHS}_{\max}= \mathsf{N}_{t+1}+ \mathsf{P}_{t+1} $. 
%%	
%%	We terminate if the following condition holds. 
%%	\[
%%	\mathsf{FP}_t  + \frac{n\lambda_2}{\lambda_1m}(\sum_{r=1}^{t}\sum_{j=1}^{m}w_{r,j} - tm)\le \mathsf{N}_{t+1}+ \mathsf{P}_{t+1}
%%	\]
%%	
%%	\begin{theorem}
%%		The lower bound on the number of samples at iteration $ t+1 $ is  $ \mathsf{FP}_t  + \frac{n\lambda_2}{\lambda_1m}(\sum_{r=1}^{t}\sum_{j=1}^{m}w_{r,j} - tm) $, the objective value at $ t+1 $ can not be minimized 
%%	\end{theorem}	
%	\begin{theorem}
%		If the number of falsified samples at iteration $ t+1 $ is more than $ \mathsf{FP}_t  + \frac{n\lambda_2}{\lambda_1m}(\sum_{r=1}^{t}\sum_{j=1}^{m}w_{r,j} - t\sum_{j=1}^{m}w_{t+1,j}) $, the new clause can not minimize the objective function. 
%	\end{theorem}
%	
%	\begin{proof}
%			Let $ z_t $ be the value of objective function at iteration $ t $. If  the new learned clause can not minimize the objective function, then the following formulation holds. 
%			\[
%			\begin{split}
%			& \qquad z_t <   z_{t+1} \Rightarrow z_t - z_{t+1} < 0\\
%			& \Rightarrow \lambda_1 \frac{\mathsf{FP}_t+\sum_{i=1}^t\mathsf{FN}_i}{n} +\lambda_2 \sum_{r=1}^t\sum_{j=1}^{m} \frac{w_{r,j}}{m \cdot t} - \lambda_1 \frac{\mathsf{FP}_{t+1}+\sum_{i=1}^{t+1}\mathsf{FN}_i}{n} -\lambda_2 \sum_{r=1}^{t+1}\sum_{j=1}^{m} \frac{w_{r,j}}{m \cdot (t+1)} <0\\
%			& \Rightarrow \lambda_1 \frac{\mathsf{FP}_t- (\mathsf{FP}_{t+1}+ \mathsf{FN}_{t+1}) }{n} + \lambda_2\frac{\sum_{r=1}^{t}\sum_{j=1}^{m}w_{r,j} - t\sum_{j=1}^{m}w_{t+1,j} }{m} <0 \\
%			& \Rightarrow  \mathsf{FP}_t  + \frac{n\lambda_2}{\lambda_1m}(\sum_{r=1}^{t}\sum_{j=1}^{m}w_{r,j} - t\sum_{j=1}^{m}w_{t+1,j})  < \mathsf{FP}_{t+1}+ \mathsf{FN}_{t+1}
%			\end{split}
%			\]
%	\end{proof}
%	
%	
%	Let us consider  $ n_t $ be the number of samples at iteration $ t $.  The objective function at the $ 1^\text{st} $ iteration is
%	\[	
%	\lambda_1 \frac{\sum \eta }{n_1} + \lambda_2 \frac{\sum w}{m}
%	\]
%	Similarly, the objective function at iteration $ 2 $ is
%	\[
%	\lambda_1 \frac{\sum \eta }{n_2} + \lambda_2 \frac{\sum w}{m}
%	\]
%	Since $ n_2 \le n_1 $, both the objective function do not put equal weight on prediction error. To put equal weight, it is required  to satisfy the following condition. 
%	\[
%	\frac{\frac{\lambda_1}{n_1}}{\frac{\lambda_2}{m}}= \frac{\frac{\lambda'_1}{n_2}}{\frac{\lambda'_2}{m}}
%	\]
%	Where $ \lambda'_1 $ and $ \lambda'_2 $ are the weights for the $ 2^\text{nd} $ partition.  Now we conclude to the following conclusion. 
%	\[
%	\frac{\lambda'_1}{\lambda'_2}= \frac{\frac{n_2\lambda_1}{n_1}}{\lambda_2}
%	\]
%	Since $ \lambda'_1  + \lambda'_2 =1$, $ \lambda'_2=1-\frac{n_2}{n_1}\lambda'_1  $
%\begin{itemize}	
%	\item When to stop
%	\item Add new term in the objective function, 
%\end{itemize}


\section{Incremental Mini-batch Rule Learning}
\label{sec:incremental_learning}
In this section, we propose a mini-batch rule learning approach that learns the  classification rule $ \Rule $ incrementally over batches.  
Since the complexity of  the MaxSAT encoding in Section~\ref{sec:encoding} depends on the size of the training set, we propose a mini-batch learning framework to reduce the number of clauses in the MaxSAT query with the aim of reducing the solution time of the query. In this approach, we select a smaller-size batch randomly from the full training set, learn a rule on the batch such that we can minimize the change in the learned rule compared to the  rule  in the previous batch while maximizing the prediction accuracy in the current batch. We repeat this process for a fixed number of iterations to learn a stable rule.   In the following, we discuss the objective function in Section~\ref{sec:obj_incremental} and then discuss the MaxSAT encoding in Section~\ref{sec:encoding_incremental}.


\subsection{Objective Function:}
\label{sec:obj_incremental}
In the incremental mini-batch learning, we design an objective function to penalize both the prediction error and the change of selection of features in the rule across consecutive batches. Let $ \tau $ be the number of iterations of the learning process and $ (\mathbf{X}',\mathbf{y}') $ be the set of  randomly chosen  samples from the training set $ (\mathbf{X},\mathbf{y}) $ of size $ n $.  We also consider $ \Rule_t $ being the $ k $-clause learned rule in the $ t $-th iteration ($ t=1, \dots, \tau $), where $ \Rule_0 $ is an empty rule. To measure the prediction error on the current batch, we consider $ \mathcal{E}_{\Rule_t} =\{(\mathbf{x},y) \in (\mathbf{X}',\mathbf{y}') | y \ne \Rule_t(\mathbf{x}) \} $ as  the set of misclassified samples from  $ (\mathbf{X}',\mathbf{y}') $. In addition, we encode the change in the rules learned in two consecutive iterations in terms of the difference of the rule-size $ |\Rule_t| - |\Rule_{t-1}| $. Given the data-fidelity parameter $ \lambda \in [0,1] $ and learning rate $ \alpha \in \mathcal{R}^+ $,  we optimize the following function at each iteration of the mini-batch setting. 



%The objective function in Eq.~\ref{eq:obj}  considers both prediction accuracy and sparsity of rules while finding the optimal assignment of noise variables and feature variables. Unlike optimizing rule-sparsity  in Eq.~\ref{eq:obj}, the new objective function for incremental approach  penalizes the different assignment of a feature variable compared against its assignment in the previous epoch. Moreover, the weight on this penalty increases gradually so that the alteration  in the assignment of a feature variable is less preferred in later epochs.  



\begin{equation}
	\label{eq:obj_incr}
	\min_{\Rule_t} \quad \frac{\lambda^{1+\frac{t-1}{\alpha (\tau-1)}}}{n} |\mathcal{E}_{\Rule_t}|+\frac{1-\lambda^{1+\frac{t-1}{\alpha (\tau-1)}}}{m k} (|\Rule_t|-|\Rule_{t-1}|)
\end{equation}


\red{$ \Delta=1-\lambda \text{ if  } \alpha \ge 0 \text{, otherwise }  \Delta=\lambda $}

\red{$\lambda$=$\lambda + \alpha \Delta \frac{t-1}{T}$, $ \alpha \in [-1,1] $}

\red{redefined}
\begin{equation}
\label{eq:obj_incr}
\min_{\Rule_t} \quad \frac{\lambda + \alpha \Delta \frac{t-1}{T}}{n} |\mathcal{E}_{\Rule_t}|+\frac{1-(\lambda + \alpha \Delta \frac{t-1}{T})}{m k} (|\Rule_t|-|\Rule_{t-1}|)
\end{equation}

In the objective function, the data-fidelity parameter $ \lambda $ has an exponent $ 1+\frac{t-1}{\alpha (\tau-1)} \in [1, 1+ \frac{1}{\alpha}] $. Since $ \lambda \in [0,1] $ and $ \alpha \in \mathcal{R}^+ $, this exponent decides  how much $ \lambda $ will decrease from its initial value as the iteration $ t $ progresses. Here $ \alpha $ decides the amount of decrease of $ \lambda $ from its initial value and acts as an inverse to the stability of the rule.  Moreover, as iteration $ t $ progresses,  the objective function tries to learn a more stable rule by putting a less penalty on the prediction error. 
In this context, the penalty on the prediction error also depends on the size of the batch since we apply the size $ n $ of the full training set to normalize the penalty on  prediction error. Intuitively, if the batch-size is close to the size of the training set, more priority is given to the prediction accuracy  and vice versa. 



\subsection{MaxSAT Encoding of Mini-batch Learning}
\label{sec:encoding_incremental}
We now discuss the MaxSAT encoding for the incremental mini-batch learning. The soft clause $ E_q $ associated with noise variables is identical to  Eq.~\ref{soft_clause_error} and the weight of this soft clause is set to $\frac{\lambda^{1+\frac{t-1}{\alpha (\tau-1)}}}{n}$.  The hard clause $ H_i $ is  identical to Eq.~\ref{hard_clause_rule_consistency} because at each iteration, we learn a $ k $-clause rule. Finally, soft clause $ S_j^i $ is modified according to the objective function as follows: 

\[
S_j^i:=
\begin{cases}
b_j^i& \text{if }  x_j \in  \clause(\Rule_{t-1},i)  \\
\neg b_j^i & \text{otherwise}
\end{cases};\qquad \mathsf{wt}(S_j^i)=\frac{1-\lambda^{1+\frac{t-1}{\alpha (\tau-1)}}}{m k}
\]

In the definition of $ S^i_j $, a feature variable $ b^i_j $ is preferred to keep its assignment in the previous iteration, otherwise the objective function is incurred a cost $ (1-\lambda^{1+\frac{t-1}{\alpha (\tau-1)}})/m k $. Intuitively,  in the optimal solution at iteration $ t $, if each feature variable is assigned to its previous assignment,  the hamming distance between two consecutive rules is zero.




%Initially each $ w_{r,j} = 0 $, hence $ S_{r,j}:= \neg w_{r,j} $ in the $ 1^\text{st} $ epoch. 


\subsection{Iterative Clause Learning in Mini-batch Setting}

We now discuss a more improved learning framework by merging both iterative clause learning approach and incremental mini-batch learning approach with an  incorporation of  feature-ranking.   In this framework, we consider a percentage of higher ranked features as described in Section~\ref{sec:feature_elimination}. Then we iteratively learn clauses on a reduced set of features, where each clause is learned in an incremental mini-batch setting. 

\label{sec:all_hypotheses}
\[
\min_{w_{r,j}} \quad \frac{\lambda^{f(t)}}{n^{(t)}} \sum_{i=1}^{n^{(t)}}\eta_i+\frac{(1-(\frac{n_i}{n}\lambda)^{f(t)})}{m k} \sum_{r=1}^k\sum_{j=1}^{m} {w^{(t)}_{r,j}- w^{(t-1)}_{r,j}} 
\]
\[
f(t)=\frac{t-1}{Tc}
\]


\red{redefined}
\[
\min_{w_{r,j}} \quad \frac{\lambda + \alpha \Delta \frac{t-1}{T}}{n^{(t)}} \sum_{i=1}^{n^{(t)}}\eta_i+\frac{(1-\frac{n_i}{n}(\lambda + \alpha \Delta \frac{t-1}{T}))}{m k} \sum_{r=1}^k\sum_{j=1}^{m} {w^{(t)}_{r,j}- w^{(t-1)}_{r,j}} 
\]







\section{More Constraints on Desired Rule:}

For the sake of interpretability, we can put additional constraints to control the rule-size and  also the preference  of an individual feature in the desired rule. For example, maximum clause-size constrains the maximum number of selected features in a clause. Let assume that, $ \sigma_i \in \{1,\dots,m\} $ is an integer  number that denotes the maximum number of selected features that the $ r $-th clause can have.\footnote{In our formulation, it is straightforward to have different  $ \sigma_i $ for different clauses.} 
\[
\sum_{j=1}^m b_j^i \le \sigma_i
\]
The above constraint is a pseudo-boolean constraint and can be encoded into CNF using an off the shelf pseudo-boolean to CNF encoder (i.e., PBEncoder~\cite{philipp2015pblib}). After encoding, we put $ \infty $ weight to each clause in the encoded CNF and append in the MaxSAT query $ Q $ as hard clauses. 

We also constrain the maximum number of selection of an individual feature in the desired rule by introducing an integer threshold $ \theta_j $ corresponding to the $ j $-th feature. 
\[
\sum_{i=1}^k b_j^i \le \theta_j
\]  
The above constraint is similarly encoded to CNF and then added to $ Q $ has hard clauses. For protected features such as age, ethnicity, sex etc., we can set corresponding $ \theta_j=0 $ so that the desired rule does not include these features in the classification rule. 




==> chapters/additional/incMLIC.tex <==
\section{ {\Framework}: }\label{sec:framework} 
\textcolor{red}{Change weight of each soft clause\\}
In this section, we present the primary contribution of this paper, {{\Framework}}, which is a MaxSAT-based incremental learning framework for interpretable classification rules. The core technical idea behind {{\Framework}} is to divide the training data into a fixed number $ p $ of partitions {and employ {\MaxSAT} based learning framework for each partition } such that the MaxSAT query constructed for partition $i$ is based on the training data for partition $i$ and the rule learned until partition $i-1$.
 To this end, we use the notation $(\mathbf{X}^i, \mathbf{y}^i) $ to refer to the training data for the $i$-th partition. We assume that  $\forall i, |\mathbf{X}^i| = |\mathbf{X}^{i-1}|$.

%The rest of the section is organized as follows: we first describe the construction of {MaxSAT} query for the  $i$-th partition  in Sect.~\ref{subsec:query} to learn CNF rules, and then discuss the discretization techniques for real-world datasets in Sect.~\ref{sec:nonbinaryfeatures}. The incrementality of {{\Framework}} gives rise to the challenge of having redundant literals in the learned rules; we address such redundancy in Sect.~\ref{sec:pruning} and finally we discuss, in Sect.~\ref{sec:dnf}, how our framework for learning CNF rules can be easily extended to learn DNF rules as well.  We provide an illustration of rule learning of {\Framework} in Appendix ~\ref{sec:example}. 


	

 
	\subsection{Construction of MaxSAT Query}\label{subsec:query}	
	


  We now discuss the construction of a  {MaxSAT} query, denoted by $Q_i$, for the  $i$-th partition ($i \in [1,p]$). To construct the {MaxSAT} query for the $i$-th partition, we assume an access to the rule learned from the  $(i-1)$-th partition (where $\R_0$ is  an empty formula). 
  
 The construction of $Q_i$ takes in four parameters: (i) $ k $, the desired number of clauses in CNF rule, (ii) $ \lambda $, the data fidelity parameter, (iii) a matrix ${\mathbf{X}^{i}} \in \{0,1\}^{n \times m}$  describing the  binary value of  $m$ features for each of    $n$ samples with $\mathbf{X}^{i}_q$ being a binary valued vector for the $ q $-th sample corresponding to feature vector $\mathbf{x} = \{x_1, x_2, \dots, x_m\}$, (iv) a label vector $\mathbf{y}^{i} \in \{0,1\}^n$ containing a class label $y^{i}_q$ for the  sample $\X^{i}_q$.   Consequently, {{\Framework}} constructs a {MaxSAT} query for the $ i $-th partition and invokes an off-the-shelf MaxSAT solver to compute the underlying rule $ \R_i $.

 

		
	{\Framework} considers two types of propositional variables: (i) feature variables and (ii) noise (classification error) variables.
%	 Feature variables are defined once for all partitiones. 
 	For the $ i $-th partition, {\Framework} formulates a classifier rule $ \R_i $ based on following intuition.  Recall, a $ k $-clause CNF rule $ \R_i=\bigwedge_{l=1}^kC_l $ is  represented as the conjunction of  $ k $ clauses where clause $ C_l $ is the disjunction of  feature variables. A  sample $ \X^i_q $ satisfies  $ C_l $ if $ \X^i_q $ has at least one similar feature whose representative variable is present in $ C_l $. If $ \X^i_q $ satisfies  $ \forall l, C_l$, then  $ \R_i(\X^i_q)=1 $ otherwise $ \R_i(\X^i_q)=0 $. Since  feature $ x_j $ can be present or not present  in each of   $ k $ clauses, {\Framework} considers $ k $  boolean variables, each denoted by $ b_j^l $ ($ l \in [1,k] $) for  feature $ x_j $ to denote its participation in the $ l $-th clause. A sample $ \X^i_q $, however, can be misclassified by $ \R_i $ i.e., $ \R_i(\X^i_q)\oplus  y_q^i =1 $.  {\Framework}  introduces  a noise variable $ \eta_q $ corresponding to  sample $ \X^i_q $ so that the assignment of $ \eta_q $ can be interpreted whether $ \X^i_q $ is misclassified by $ \R_i $ or not.  Hence the key idea of {{\Framework}} for learning the $ i $-th partition is to define a {MaxSAT} query over $k \times m + n$ propositional variables, denoted by $\{ b_{1}^{1}, b_{2}^{1}, \dots ,b_{m}^{1}, \dots ,b_{m}^{k}, \eta_1, \dots ,\eta_n\}$.   The {\MaxSAT} query of {\Framework} consists of the following three sets of constraints:
  

 	
	\begin{enumerate}
		
		\item Since our objective is to find sparser rules, the default objective of  {\Framework} would be to add a constraint to falsify as many $ b_j^l $  as possible. 	As noted earlier,  rule $\Rule_{i-1}$ from the $(i-1)$-th partition plays an important role in the construction of MaxSAT 
		constraints of the $i$-th partition. Therefore,   if $x_{j} \in \clause(R_{i-1},l)$, {\Framework} would deviate from its default behavior by adding a constraint to keep the corresponding literal $ true $ in the optimal assignment.  The weight corresponding to this clause is $ 1 $. We formalize our discussion as follows:
	\begin{equation*}
	V^l_j:= 
	\begin{cases}
	b^l_j&\quad \text{if }  x_{j} \in \clause(\R_{i-1},l)\\
	\neg b^l_j&\quad \text{otherwise } \\
	\end{cases}
	;\quad  W(V^l_j)= 1
	\label{eq:constraint-v}
	\end{equation*}
		\item We use noise variables to handle mis-classifications and therefore, {\Framework} tries to falsify as many   noise variables as possible. Since data fidelity parameter $ \lambda $ is proportionate to accuracy, {\Framework} puts $ \lambda $ weight to each following soft  clause. 

		\begin{equation*}
		N_q:= (\neg \eta_q ); \qquad \qquad W(N_q) = \lambda
		\label{eq:constraint_two}
		\end{equation*}
		%		Here $N_i $ is also a soft clause. 
		
		\item 
		Let $\mathbf{B}_{l} = \{b^{l}_{j} \mid j \in [1,m] \}$. 
		Here we provide the third set of constraints of {\Framework}. 
		\begin{equation*}
		D_q:= (\neg \eta_q \rightarrow ( y_q \leftrightarrow \bigwedge_{l=1}^{k} ({\mathbf{X}_q} \vee {\mathbf{B}_{l}})));    W(D_q) = \infty
		\label{eq:constraint_three}	
		\end{equation*}
		Every hard clause $D_q$  can be interpreted as follows. If $\eta_q$ is assigned to \textit{false} ($ \neg \eta_q = true$) then ${y}^i_q = \R_i(\X^i_q)=\bigwedge_{l=1}^{k} ({\mathbf{X}_q} \vee {\mathbf{B}_{l}})$.  The operator ``$\vee  $'' is defined in Sect. \ref{sec:preliminaries}.  
		
		%		We are not showing in details how $ D_i $ can be encoded into CNF forms using standard procedure. We refer \cite{MM18} for detailed description.
		
		
	\end{enumerate}
	Finally, the set of constraints $Q_i$ for  the $ i $-th partition constructed by {{\Framework}} is defined as follows:
	\begin{equation*}
	\label{eq:constraint-imli}
	Q_i :=  \bigwedge_{j=1, l = 1}^{j=m,l=k} V^l_j \wedge \bigwedge_{q=1}^{n} N_q \wedge \bigwedge_{q=1}^{n} D_q
	\end{equation*} 
	
	Next, we extract $\Rule_i$ from the solution of $Q_i$ as follows. 
	\begin{construction}
		Let $\sigma^* = \MaxSAT(Q_i,W)$, then $x_j \in {\clause(\Rule_i,l)}$ iff $\sigma^*(b_{j}^{l}) = 1$.
	\end{construction}
	In the rest of the manuscript, we will use $\Rule$ to denote $\Rule_{p}$.  
	\subsection{Beyond Binary Features}\label{sec:nonbinaryfeatures}
	

	We have considered that the feature value of a training sample is binary. Real-world  datasets, however,  contain categorical, real-valued or numerical features. We use the standard discretization technique to convert categorical and continuous (real or integer value) features to boolean features. We use  {\em one hot encoding} to convert categorical features to binary features by introducing a boolean vector  with the cardinality equal to the number of distinct categories of individual categorical features.
	\begin{example}
		\label{ex:bin_categorical}
		Consider a categorical feature with three categories: ``red'', ``green'', ``'yellow''. One hot encoding would convert this feature to three binary variables, which take values $ 100 $, $ 010 $, and $ 001 $ for the three categories.
	\end{example}
	
	 Furthermore, we can discretize the continuous-valued features into  binary features by comparing the feature value to  a collection of  thresholds within range and introducing  a boolean feature vector with cardinality proportional to the number of considered threshold.
Specifically, for a continuous feature $ x_c $ we consider a number of thresholds $ \{\tau_1,\dots,\tau_t\}$ where $  \tau_i < \tau_{i+1}  $ and define two separate Boolean features $ I[x_c \ge \tau_i] $ and $ I[x_c < \tau_i] $ for each $ \tau_i $. 
	We present the following definitions based on the discretization of  continuous features.
	
		 	\begin{definition}
		 		$ tval(b): b \rightarrow \tau $ is a function over boolean variables corresponding to discretized binary features (from a continuous feature) and outputs the compared threshold value. 
		 	\end{definition}
		 	
		 	\begin{definition}
		 		$ op(b): b \rightarrow \{\ge , <\} $ is a function over boolean variables corresponding to discretized binary features (from a continuous feature) and outputs the comparison operator between continuous feature value and $ tval(b) $. 
		 	\end{definition}
		 	
		 	\begin{definition}
		 		$ siblings(b_i, b_j): (b_i, b_j) \rightarrow \{true, false\} $ is a function over pair of  boolean variables $ b_i,b_j $ and outputs $ true $ if the boolean features corresponding to $ b_i,b_j $ are constructed by discretizing the same continuous feature  
		 		and  
		 		$ op(b_i)=op(b_j) $.
		 	\end{definition}
	 	
%	 	\begin{example}
%	 		\label{ex:bin_categorical}
%	 		Consider a categorical feature with three categories: ``red'', ``green'', ``'yellow''. One hot encoding would convert this feature to three binary variables, which take values $ 100 $, $ 010 $, and $ 001 $ for the three categories.
%	 	\end{example}
	 	\begin{example}
	 		\label{ex:bin-continuous}
	 		Consider  a  continuous feature $ x_c $ with range $  (0,100) $ and three thresholds $ \{25,50,75\} $ associated with this feature.  $ \Framework $ introduces $ 6 $ new boolean features   $ \{ x_1: I[x_c\ge 25],x_2: I[x_c\ge 50], x_3:I[x_c\ge 75], x_4:I[x_c< 25], x_5:I[x_c< 50],x_6:I[x_c < 75]\} $. Following this discretization technique,  the binary feature vector  of a sample  with   feature value $ x_c=37.5 $ is  $ 100011 $, because among the $6  $ introduced boolean features $ x_1:I[ 37.5 \ge 25 ]=1$, $ x_5:I[37.5 < 50]=1 $, and $x_6:I[ 37.5 < 75]=1 $.
	 		
	 		
	 	\end{example}
	 	
	 	\begin{example}
	 		\label{ex:prune}
	 		In Example \ref{ex:bin-continuous}, $ b_i $ is a boolean variable corresponding to feature $ x_i $. Now $ tval(b_1)=25$, $ op(b_1)=\text{``}\ge\text{''}$, $ siblings(b_1,b_2)=true, $ and $ siblings(b_1,b_4)=false $. 
	 	\end{example}
 	
	
	
		



	\subsection{Redundancy Removal}\label{sec:pruning}
	Given the incremental procedure of learning {\Rule} where the constraints for the $i$-th partition are influenced from the rule learned until the $(i-1)$-th partition, one key challenge is to address potential redundancy in the learned rules. In particular, we observe that redundancy manifests itself in binary features corresponding to continuous-valued features as the $(i-1)$-th partition  might suggest inclusion of feature  $ I[x_c < \tau_u] $ while the $ i $-th partition  also suggests inclusion of feature $ I[x_c < \tau_v] $ where $\tau_u \ne \tau_v$. To this end, we present Algorithm \ref{alg:imli-RRL} to remove redundant literals. 

	\begin{algorithm}
		\caption{Remove Redundancy}\label{alg:imli-RRL}
		\begin{algorithmic}[1]
			\Procedure{removeRedundantLiterals}{$\R$}
			\For{each  clause $ C_l $ of $ \R $} 
			\For{ each pair $ \langle b_i^l,b_j^l \rangle $  where   $ \sigma(b_i^l)=\sigma(b_j^l)=1$,   $siblings(b_i^l,b_j^l)=true $, and $ tval(b_i^l) < tval(b_j^l) $ }
			\If {$op(b_i^l)=op(b_j^l)=\text{``}\ge \text{''} $}
			\State  $ \R'=\R[\sigma(b_j^l)\mapsto0] $ \Comment{$ b_j^l $ is redundant}
			\Else \State $ \R'=\R[\sigma(b_i^l)\mapsto0] $
			\EndIf
			\EndFor
			\EndFor
			\State \Return $ \R' $
			\EndProcedure
		\end{algorithmic}
	\end{algorithm}




	\begin{lemma}
		 $ |\R'| \le |\R| $ and $ \R' $ is equivalent to $ \R $. 
		
		\label{lm:adjustment_of_rule_size}
	\end{lemma}
\begin{proof}
	\label{prf:prune}
	%		Removed due to the brevity of presentation.
	The case  $ |\R'|=|R| $ is trivial because no literal is removed from $ \R' $, and $ \R' $ is equivalent to  $ \R $.
	
	
	When $ |\R'| < |\R| $, $ \exists \langle b_i^l,b_j^l \rangle $  where $  l \in [1,k] $,    $siblings(b_i^l,b_j^l)=true $, $ tval(b_i^l) < tval(b_j^l) $, and $ x_c $ is the considered continuous feature. 
	
	Suppose  $op(b_i^l)=op(b_j^l)=\text{``}\ge \text{''} $. Consider two sets of real number: $ S_i= \{x_i: x_i \ge  tval(b_i^l)\} $ and $ S_j=\{x_j: x_j \ge  tval(b_j^l)\} $. As $ \R $ is in CNF,  $ \R $ checks $ I[x_c \in S_i \cup S_j] $  to classify  $ \forall q,\mathbf{X}_q  $. Here $ S_i \cup S_j = S_i $, so $ b_j^l $ can be pruned.
	
	We can prove similarly when $op(b_i^l)=op(b_j^l)=\text{``}< \text{''} $.
	
	Therefore, $ |\R'| \le |\R| $ and $ \R' $ is equivalent to $ \R $.
	
\end{proof}

	
		
		

	\subsection{Learning DNF Rules}
	\label{sec:dnf}


			Primarily we focus on learning rule $ \R $ which is in CNF form. We can also apply incremental technique for learning DNF rules.   Suppose, we want to learn a rule $ y=S(x) $ where $ S(x) $ is expressible in DNF. We show that $ y = S(x) \leftrightarrow \neg (y=\neg S(x)) $. Here $ \neg S(x) $ is in CNF.  Therefore, to learn DNF rule $ S(x) $, we simply call {\Framework} with $ \neg \mathbf{y} $ as input  for all $ p $ batches, learn CNF rule, and finally
	negate the learned rule.  Hence Algorithm \ref{alg:imli-RRL} can be directly applied.
	\begin{example}
		\label{ex:dnf_rule}
		``$( \text{is Male}\vee \text{Age}<\text{50})\wedge(\text{Education}=\text{Graduate}\vee\text{Income}\ge\text{1500}) $''\textemdash rule is  learned for negated class label. The resultant DNF rule is  ``$ (\text{is not Male}\wedge  \text{Age}\ge\text{50}) \vee (\text{Education} \ne \text{Graduate}\wedge\text{Income}<\text{1500} )$'' 
	\end{example}

		

==> chapters/additional/proposed_improvement.tex <==
\section{Convert to MDP}
	
	\textcolor{red}{change $ \tau $ in previous section}

	Markov decision process is a $ 4 $-tuple $ (S,A,P_a,R_a) $ where 
	
	\begin{itemize}
		\item $ S $ is a finite set of states.
		\item $ A $ is a finite set of actions (alternately, $ A_s $ is the finite set of actions available from state $ s $).
		\item $ P_a(s,s')=\probability(s_{i+1}=s' | s_i=s, a_i=a) $ is the probability that action $ a $ in state $ s $ at time $ i $ will lead to state $ s' $ at time $ i+1 $. 
		\item $ R_a(s,s') $ is the immediate reward (or expected immediate reward) after transitioning from state $ s $ to $ s' $, due to action $ a $.
	\end{itemize}

	We can fit our problem as a Markov decision process as follows.
	
	\begin{itemize}
		\item We have $ \tau $ states, which is equal to the number of partitions. In state $ s_i $, we learn $ \Rule_i $. 
		\item From  each state $ s_i $, we can take two actions,  $\{ a_0,a_1 \} $ where $ a_0= \text{keep rule } \Rule_{i} $ and $  a_1 =  \text{ revert to rule } \Rule_{i-1} $
		\item  Let assume that, $ z_{i} $ is the cost function after solving the MaxSAT query $ Q_i $ in state $ s_i $. We can calculate $ z_i $ using Eq~\ref{eq:cost}.   We define transition probability as follows. 
			\[
			\begin{split}
			&P_{a_0}(s_i,s_{i+1})= \frac{1}{1+e^{z_i - z_{i-1}}}\\
			&P_{a_1}(s_i,s_{i+1})= \frac{1}{1+e^{z_{i-1} - z_i}}
			\end{split}
			\]
		Since we minimize the cost function in Eq~\ref{eq:cost}, $  P_{a_0}(s_i,s_{i+1}) > P_{a_1}(s_i,s_{i+1}) $, when $ z_i < z_{i-1} $.
		\item We define reward probability as follows. 
		\[
		\begin{split}
			&R_{a_0}(s_i,s_{i+1})=-z_i\\
			&R_{a_1}(s_i,s_{i+1})= - z_{i-1}			
		\end{split}
		\]
	\end{itemize}
	
	
	
%	We can consider a Markov Decision Process. In state $ S_i $, we learn rule $ R_i $. We take two actions from state $ S_i $ to $ S_{i+1} $. We can either keep rule $ R_i $, or revert to $ R_{i-1} $.  
%
%	
%	Now we have two choices: either keep rule $ \Rule_{i} $ or revert to $ \Rule_{i-1} $. We make the decision based on the value of $ z_{i} $ and $ z_{i-1} $.  We consider a probability distribution over the difference between $ z_i $ and $ z_{i-1} $ as follows. 
	
	

==> chapters/review-response.tex <==
We thank the reviewers for their constructive feedback and suggestions on improving the paper. We address the comments below and reflect them in the revised paper. 

\vspace{1em}
\noindent\textbf{Response to Reviewer A}

In addition to learning logical rules from data, our interpretable classifier {\framework} can also serve as an alternative approach to decompositional and pedagogical extractors of logical rules for black-box classifiers such as neural networks and SVMs. To this end, we can deploy {\framework} as an efficient rule-learner to learn interpretable rules given input-output examples from an existing black-box classifier. We have elaborated on this in the related works (last paragraph in Section 2).

In our experiments, we focus on datasets, where input variables are interpretable to humans. In contrast to applications such as NLP and computer vision, interpretable domains typically consider a limited number of variables, where each variable refers to a Boolean abstraction of a complex feature representation. However, {\framework} can still handle classifications with thousands of variables, and it can potentially scale beyond that.

{\framework} can be extended to more flexible interpretability objectives than the simplified `accuracy vs sparsity' objective. We have elaborated on this in Section 5.4. 

For experimental comparisons with pure sub-symbolic  models, the reviewer has not provided any reference. We, however, agree with the reviewer that {\framework} can be applied as a logical knowledge extractor given input-output examples. In this paper, we focus on improving the scalability of a rule-learner while achieving competitive accuracy and rule sparsity. The experiment on applying {\framework} as a logical knowledge extractor is beyond the scope of the current work. 

\vspace{1em}
\noindent\textbf{Response to Reviewer B} 

In the introduction, we have placed an interpretable classification rule in CNF for the WDBC dataset, which decides on predicting the type of a tumor cell. According to the suggestion of the reviewer, we have added interpretable rules for all datasets at the end of the paper (in the Appendix). 

We thank the reviewer for the edit in section 3.1. We have proofread all formulas in the revised version.
